Addressing $H_0$ tension with emergent dark radiation in unitary gravity

We propose a one-parameter extension to $\Lambda$CDM, expected to strongly affect cosmological tensions. An effective dark radiation component in the early universe redshifts away as hot dark matter, then quintessence, tracking the dominant equation-of-state parameter and leaving a falsifiable torsion field in the current epoch. This picture results from a new Poincar\'{e} gauge theory (PGT), one of the most promising among the latest batch of 58 PGTs found to be both power-counting renormalisable and free from ghosts and tachyons. We systematically categorise the cosmologies of 33 of these PGTs, as special cases of the most general parity-preserving, Ostrogradsky-stable PGT with a purely Yang-Mills action. The theory we consider contains two propagating massless gravitons, which may be $J^P=2^+$ (long-range gravitation and gravitational waves). A conspiracy among the coupling constants eliminates the spatial curvature $k\in\{\pm 1,0\}$ from the field equations. We show that this `$k$-screening' is not restricted to conformal gravity theories. The flat Friedmann equations are then emergent, with potentially tension-resolving freedom at the early scale-invariant epoch that reliably gives way to an attractor-like state of modern $\Lambda$CDM evolution. We compare with related theories and promising special cases, such as $k$-screened theories with negative-definite effective $k$, and more traditional theories with effective $\Lambda$ and a $J^P=0^-$ massive graviton (dark matter candidate). As a bonus, we analyse similarly constrained actions in the new extended Weyl gauge theory (eWGT). We show that in cosmology, PGT and eWGT span exactly the same classical phenomenology up to a linear map between their coupling constants, hinting at a deeper relationship between the two.

==> sa0_base.tex <==
y=({\it Q0}-{\frac {{M}^{2} \left( 3\,{{\it Q0}}^{2}-1 \right) \sqrt {3}}{16\,R}}x+{\frac {{M}^{4} \left( 162
\,{{\it Q0}}^{4}-15\,{{\it Q0}}^{2}-13 \right) }{1536\,{\it Q0}\,{R}^{2}}}{x}^{2}-{\frac { \left( 3\,{{\it Q0
}}^{2}-1 \right) {M}^{6} \left( 2916\,{{\it Q0}}^{4}+837\,{{\it Q0}}^{2}+299 \right) \sqrt {3}}{442368\,{R}^{
3}{{\it Q0}}^{2}}}{x}^{3}+{\frac {131220\,{M}^{8}{{\it Q0}}^{8}-1422\,{M}^{8}{{\it Q0}}^{4}-294912\,{L}^{2}{R
}^{6}{{\it Q0}}^{2}+2595\,{M}^{8}{{\it Q0}}^{2}+98304\,{L}^{2}{R}^{6}-2327\,{M}^{8}}{11796480\,{R}^{4}{{\it 
Q0}}^{3}}}{x}^{4}+{\frac { \left( -11809800\,{M}^{8}{{\it Q0}}^{8}-4483350\,{M}^{8}{{\it Q0}}^{6}-1439775\,{M
}^{8}{{\it Q0}}^{4}-388068\,{M}^{8}{{\it Q0}}^{2}+6684672\,{L}^{2}{R}^{6}-361231\,{M}^{8} \right)  \left( 3\,
{{\it Q0}}^{2}-1 \right) {M}^{2}\sqrt {3}}{16986931200\,{R}^{5}{{\it Q0}}^{4}}}{x}^{5})

